Unbiased mm-wave Line Surveys of TW Hya and V4046 Sgr: The Enhanced C2H and CN Abundances of Evolved Protoplanetary Disks

We have conducted the first comprehensive mm-wave molecular emission line surveys of the evolved circumstellar disks orbiting the nearby T Tauri stars TW Hya and V4046 Sgr AB. Both disks are known to retain significant residual gaseous components, despite the advanced ages of their host stars. Our unbiased broad-band radio spectral surveys of the TW Hya and V4046 Sgr disks were performed with the Atacama Pathfinder Experiment (APEX) 12 meter telescope and are intended to yield a complete census of bright molecular emission lines in the range 275-357 GHz (1.1-0.85 mm). We find that lines of 12CO, 13CO, HCN, CN, and C2H, all of which lie in the higher-frequency range, constitute the strongest molecular emission from both disks in the spectral region surveyed. The molecule C2H is detected here for the first time in both disks, as is CS in the TW Hya disk. The survey results also include the first measurements of the full suite of hyperfine transitions of CN N=3-2 and C2H N=4-3 in both disks. Modeling of these CN and C2H hyperfine complexes in the spectrum of TW Hya indicates that the emission from both species is optically thick and may originate from very cold disk regions. It furthermore appears that the fractional abundances of CN and C2H are significantly enhanced in these evolved protoplanetary disks relative to the fractional abundances of the same molecules in the environments of deeply embedded protostars.

==> PierreLatexDefs.tex <==
\def\phb#1{#1} %\textbf{#1}}
\def\reac#1#2{\begin{equation}\label{r:r#1}\ce{#2}\end{equation}}
\def\reacnn#1{\[\ce{#1}\]}
\def\refreac#1{(\ref{r:r#1})}
\def\abS{\ensuremath{[\ce{S}]_{\rm tot}}}
\def\ab#1{\ensuremath{[\ce{#1}]}}
\def\fch2{\ensuremath{f_{\ce{CH2}}}}
\def\fhcn{\ensuremath{f_{\rm HCN}}}
\def\fhnc{\ensuremath{f_{\rm HNC}}}
\def\fcn{\ensuremath{f_{\rm CN}}}
\def\fifn{\ensuremath{\ce{^{15}N}}}
\def\fif{$^{15}$}
\def\fifnp{\ensuremath{\ce{^{15}N+}}}
\def\foun{\ensuremath{\ce{$^{14}$N}}}
\def\fifno{\ensuremath{\ce{$^{15}$NO}}}
\def\cfifn{\ensuremath{\ce{C$^{15}$N}}}
\def\nfifn{\ensuremath{\ce{N$^{15}$N}}}
\def\cfoun{\ensuremath{\ce{C$^{14}$N}}}
\def\hcfifn{\ensuremath{\ce{HC$^{15}$N}}}
\def\hfifnc{\ensuremath{\ce{H$^{15}$NC}}}
\def\conv{\ensuremath{{\cal N}\ul}}
\def\tauul{\ensuremath{\tau_{ul}}}
\def\ul{\ensuremath{{_{ul}}}}
\def\tul{\ensuremath{T_{ul}}}
\def\aul{\ensuremath{A_{ul}}}
\def\gup{\ensuremath{g_u}}
\def\Ntot{\ensuremath{N_{\rm tot}}}
\def\qpart{\ensuremath{Q_{\rm exc}}}
\def\qtot{\ensuremath{Q_{\rm tot}}}
\def\qrot{\ensuremath{Q_{\rm rot}}}
\def\rr{\ensuremath{\thcn/\cfifn}}
\def\rrr{\ensuremath{\cfoun/\cfifn}}
\def\nratio {\ensuremath{{\foun/\fifn}}}
\def\nhhd   {\ensuremath{\rm NH_2D}}
\def\nnhp   {\ensuremath{\rm N_2H^+}}
\def\NH    {\ensuremath{\rm NH}}
\def\NHH    {\ensuremath{\rm NH_2}}
\def\nhhh   {\ensuremath{\rm NH_3}}
\def\fifnhh {\ensuremath{\rm ^{15}NH_2}}
\def\fifnhhh{\ensuremath{\rm ^{15}NH_3}}
\def\fifnnhp{\ensuremath{\rm ^{15}NNH^+}}
\def\nfifnhp{\ensuremath{\rm N^{15}NH^+}}
\def\perth{\ensuremath{\hbox{$\,^0\!/_{00}$}}}
\def\perth{\textperthousand}
\def\jnu{\ensuremath{J_\nu}}
\def\tpeak{\ensuremath{T_{\rm mb, 0}}}
\def\tpeak{\ensuremath{T_0}}
\def\aff{\ensuremath{A_{FF'}}}
\def\fbeam{\ensuremath{f_{\rm dilution}}}

